Towards Secrecy-Aware Attacks Against Trust Prediction in Signed Social Networks

Signed social networks are widely used to model the trust relationships among online users in security-sensitive systems such as cryptocurrency trading platforms, where trust prediction plays a critical role. In this paper, we investigate how attackers could mislead trust prediction by secretly manipulating signed networks. To this end, we first design effective poisoning attacks against representative trust prediction models. The attacks are formulated as hard bi-level optimization problems, for which we propose several efficient approximation solutions. However, the resulting basic attacks would severely change the structural semantics (in particular, both local and global balance properties) of a signed network, which makes the attacks prone to be detected by the powerful attack detectors we designed. Given this, we further refine the basic attacks by integrating some conflicting metrics as penalty terms into the objective function. The refined attacks become secrecy-aware, i.e., they can successfully evade attack detectors with high probability while sacrificing little attack performance. We conduct comprehensive experiments to demonstrate that the basic attacks can severely disrupt trust prediction but could be easily detected, and the refined attacks perform almost equally well while evading detection. Overall, our results significantly advance the knowledge in designing more practical attacks, reflecting more realistic threats to current trust prediction models. Moreover, the results also provide valuable insights and guidance for building up robust trust prediction systems.

==> citation.tex <==


@inproceedings{huang2021sdgnn,
	title={SDGNN: Learning node representation for signed directed networks},
	author={Huang, Junjie and Shen, Huawei and Hou, Liang and Cheng, Xueqi},
	booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
	volume={35},
	number={1},
	pages={196--203},
	year={2021}
}

@article{ER,
  title={On the evolution of random graphs},
  author={Erd{\H{o}}s, Paul and R{\'e}nyi, Alfr{\'e}d and others},
  journal={Publ. Math. Inst. Hung. Acad. Sci},
  volume={5},
  number={1},
  pages={17--60},
  year={1960}
}

@inproceedings{zhou2020robust,
  title={Robust Collective Classification against Structural Attacks},
  author={Zhou, Kai and Vorobeychik, Yevgeniy},
  booktitle={Conference on Uncertainty in Artificial Intelligence},
  pages={250--259},
  year={2020},
  organization={PMLR}
}

@book{MatrixExp, place={Cambridge}, title={Topics in Matrix Analysis}, publisher={Cambridge University Press}, author={Horn, Roger A. and Johnson, Charles R.}, year={1991}}

@book{zhang2011matrix,
	title={Matrix theory: basic results and techniques},
	author={Zhang, Fuzhen},
	year={2011},
	publisher={Springer}
}

@article{tsvd,
	title={The approximation of one matrix by another of lower rank},
	author={Eckart, Carl and Young, Gale},
	journal={Psychometrika},
	volume={1},
	number={3},
	pages={211--218},
	year={1936},
	publisher={Springer}
}

@INPROCEEDINGS{attacksignsimilarity,
	author={Godziszewski, Micha{\l} Tomasz and Michalak, Tomasz P and Waniek, Marcin and Rahwan, Talal and Zhou, Kai and Zhu, Yulin},
	booktitle={2021 IEEE International Conference on Data Mining (ICDM)}, 
	title={Attacking Similarity-Based Sign Prediction}, 
	year={2021}}

@InProceedings{RLS2V,
	title = 	 {Adversarial Attack on Graph Structured Data},
	author =       {Dai, Hanjun and Li, Hui and Tian, Tian and Huang, Xin and Wang, Lin and Zhu, Jun and Song, Le},
	booktitle = 	 {Proceedings of the 35th International Conference on Machine Learning},
	pages = 	 {1115--1124},
	year = 	 {2018},
	editor = 	 {Dy, Jennifer and Krause, Andreas},
	volume = 	 {80},
	series = 	 {Proceedings of Machine Learning Research},
	month = 	 {10--15 Jul},
	publisher =    {PMLR},
	pdf = 	 {http://proceedings.mlr.press/v80/dai18b/dai18b.pdf},
	url = 	 {https://proceedings.mlr.press/v80/dai18b.html},
	abstract = 	 {Deep learning on graph structures has shown exciting results in various applications. However, few attentions have been paid to the robustness of such models, in contrast to numerous research work for image or text adversarial attack and defense. In this paper, we focus on the adversarial attacks that fool deep learning models by modifying the combinatorial structure of data. We first propose a reinforcement learning based attack method that learns the generalizable attack policy, while only requiring prediction labels from the target classifier. We further propose attack methods based on genetic algorithms and gradient descent in the scenario where additional prediction confidence or gradients are available. We use both synthetic and real-world data to show that, a family of Graph Neural Network models are vulnerable to these attacks, in both graph-level and node-level classification tasks. We also show such attacks can be used to diagnose the learned classifiers.}
}

@inproceedings{hrat,
	author = {Zhao, Kaifa and Zhou, Hao and Zhu, Yulin and Zhan, Xian and Zhou, Kai and Li, Jianfeng and Yu, Le and Yuan, Wei and Luo, Xiapu},
	title = {Structural Attack against Graph Based Android Malware Detection},
	year = {2021},
	isbn = {9781450384544},
	publisher = {Association for Computing Machinery},
	address = {New York, NY, USA},
	url = {https://doi.org/10.1145/3460120.3485387},
	doi = {10.1145/3460120.3485387},
	abstract = {Malware detection techniques achieve great success with deeper insight into the semantics of malware. Among existing detection techniques, function call graph (FCG) based methods achieve promising performance due to their prominent representations of malware's functionalities. Meanwhile, recent adversarial attacks not only perturb feature vectors to deceive classifiers (i.e., feature-space attacks) but also investigate how to generate real evasive malware (i.e., problem-space attacks). However, existing problem-space attacks are limited due to their inconsistent transformations between feature space and problem space.In this paper, we propose the first structural attack against graph-based Android malware detection techniques, which addresses the inverse-transformation problem [1] between feature-space attacks and problem-space attacks. We design a Heuristic optimization model integrated with Reinforcement learning framework to optimize our structural ATtack (HRAT). HRAT includes four types of graph modifications (i.e., inserting and deleting nodes, adding edges and rewiring) that correspond to four manipulations on apps (i.e., inserting and deleting methods, adding call relation, rewiring). Through extensive experiments on over 30k Android apps, HRAT demonstrates outstanding attack performance on both feature space (over 90% attack success rate) and problem space (up to 100% attack success rate in most cases). Besides, the experiment results show that combing multiple attack behaviors strategically makes the attack more effective and efficient.},
	booktitle = {Proceedings of the 2021 ACM SIGSAC Conference on Computer and Communications Security},
	pages = {3218–3235},
	numpages = {18},
	keywords = {structural attack, android malware detection, function call graph},
	location = {Virtual Event, Republic of Korea},
	series = {CCS '21}
}


@misc{zhu2021binarizedattack,
	title={BinarizedAttack: Structural Poisoning Attacks to Graph-based Anomaly Detection}, 
	author={Yulin Zhu and Yuni Lai and Kaifa Zhao and Xiapu Luo and Mingquan Yuan and Jian Ren and Kai Zhou},
	year={2021},
	eprint={2106.09989},
	archivePrefix={arXiv},
	primaryClass={cs.LG}
}

@inproceedings{sdgnn,
	title={SDGNN: Learning Node Representation for Signed Directed Networks},
	author={Huang, Junjie and Shen, Huawei and Hou, Liang and Cheng, Xueqi},
	booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
	volume={35},
	number={1},
	pages={196--203},
	year={2021}
}

@inproceedings{edgehist,
	author = {Sugiyama, Mahito and Borgwardt, Karsten M.},
	title = {Halting in Random Walk Kernels},
	year = {2015},
	publisher = {MIT Press},
	address = {Cambridge, MA, USA},
	abstract = {Random walk kernels measure graph similarity by counting matching walks in two graphs. In their most popular form of geometric random walk kernels, longer walks of length k are downweighted by a factor of λk (λ < 1) to ensure convergence of the corresponding geometric series. We know from the field of link prediction that this downweighting often leads to a phenomenon referred to as halting: Longer walks are downweighted so much that the similarity score is completely dominated by the comparison of walks of length 1. This is a naive kernel between edges and vertices. We theoretically show that halting may occur in geometric random walk kernels. We also empirically quantify its impact in simulated datasets and popular graph classification benchmark datasets. Our findings promise to be instrumental in future graph kernel development and applications of random walk kernels.},
	booktitle = {Proceedings of the 28th International Conference on Neural Information Processing Systems - Volume 1},
	pages = {1639–1647},
	numpages = {9},
	location = {Montreal, Canada},
	series = {NIPS'15}
}

@article{tSNE,
	author  = {Laurens van der Maaten and Geoffrey Hinton},
	title   = {Visualizing Data using t-SNE},
	journal = {Journal of Machine Learning Research},
	year    = {2008},
	volume  = {9},
	number  = {86},
	pages   = {2579-2605},
	url     = {http://jmlr.org/papers/v9/vandermaaten08a.html}
}

@article{RBF,
	title={A primer on kernel methods},
	author={Vert, Jean-Philippe and Tsuda, Koji and Sch{\"o}lkopf, Bernhard},
	journal={Kernel methods in computational biology},
	volume={47},
	pages={35--70},
	year={2004},
	publisher={MIT press Cambridge, MA}
}

@inbook{autocovariance,
	author = {Huang, Zexi and Silva, Arlei and Singh, Ambuj},
	title = {A Broader Picture of Random-Walk Based Graph Embedding},
	year = {2021},
	isbn = {9781450383325},
	publisher = {Association for Computing Machinery},
	address = {New York, NY, USA},
	url = {https://doi.org/10.1145/3447548.3467300},
	abstract = {Graph embedding based on random-walks supports effective solutions for many graph-related downstream tasks. However, the abundance of embedding literature has made it increasingly difficult to compare existing methods and to identify opportunities to advance the state-of-the-art. Meanwhile, existing work has left several fundamental questions---such as how embeddings capture different structural scales and how they should be applied for effective link prediction---unanswered. This paper addresses these challenges with an analytical framework for random-walk based graph embedding that consists of three components: a random-walk process, a similarity function, and an embedding algorithm. Our framework not only categorizes many existing approaches but naturally motivates new ones. With it, we illustrate novel ways to incorporate embeddings at multiple scales to improve downstream task performance. We also show that embeddings based on autocovariance similarity, when paired with dot product ranking for link prediction, outperform state-of-the-art methods based on Pointwise Mutual Information similarity by up to 100%.},
	booktitle = {Proceedings of the 27th ACM SIGKDD Conference on Knowledge Discovery & Data Mining},
	pages = {685–695},
	numpages = {11}
}

@inproceedings{graph_classify,
  title={An end-to-end deep learning architecture for graph classification},
  author={Zhang, Muhan and Cui, Zhicheng and Neumann, Marion and Chen, Yixin},
  booktitle={Thirty-Second AAAI Conference on Artificial Intelligence},
  year={2018}
}

@inproceedings{ocsvm,
  title={Support vector method for novelty detection.},
  author={Sch{\"o}lkopf, Bernhard and Williamson, Robert C and Smola, Alexander J and Shawe-Taylor, John and Platt, John C and others},
  booktitle={NIPS},
  volume={12},
  pages={582--588},
  year={1999},
  organization={Citeseer}
}

@inproceedings{pole,
	author = {Huang, Zexi and Silva, Arlei and Singh, Ambuj},
	title = {POLE: Polarized Embedding for Signed Networks},
	booktitle = {WSDM},
	year = {2022}
}

@inproceedings{10.1145/3336191.3371789,
	author = {Entezari, Negin and Al-Sayouri, Saba A. and Darvishzadeh, Amirali and Papalexakis, Evangelos E.},
	title = {All You Need Is Low (Rank): Defending Against Adversarial Attacks on Graphs},
	year = {2020},
	isbn = {9781450368223},
	publisher = {Association for Computing Machinery},
	address = {New York, NY, USA},
	url = {https://doi.org/10.1145/3336191.3371789},
	doi = {10.1145/3336191.3371789},
	booktitle = {Proceedings of the 13th International Conference on Web Search and Data Mining},
	pages = {169–177},
	numpages = {9},
	keywords = {graph representation learning, graph mining, graph convolutional networks, adversarial machine learning, tensors},
	location = {Houston, TX, USA},
	series = {WSDM '20}
}

@inproceedings{zhang2020gnnguard,
	title     = {GNNGuard: Defending Graph Neural Networks against Adversarial Attacks},
	author    = {Zhang, Xiang and Zitnik, Marinka},
	booktitle = {Proceedings of Neural Information Processing Systems, NeurIPS},
	year      = {2020}
}

@inproceedings{tang2020transferring,
	title={Transferring robustness for graph neural network against poisoning attacks},
	author={Tang, Xianfeng and Li, Yandong and Sun, Yiwei and Yao, Huaxiu and Mitra, Prasenjit and Wang, Suhang},
	booktitle={Proceedings of the 13th International Conference on Web Search and Data Mining},
	pages={600--608},
	year={2020}
}

@inproceedings{gcn,
	author    = {Thomas N. Kipf and
	Max Welling},
	title     = {Semi-Supervised Classification with Graph Convolutional Networks},
	booktitle = {5th International Conference on Learning Representations, {ICLR} 2017,
	Toulon, France, April 24-26, 2017, Conference Track Proceedings},
	publisher = {OpenReview.net},
	year      = {2017},
	url       = {https://openreview.net/forum?id=SJU4ayYgl},
	timestamp = {Thu, 25 Jul 2019 14:25:55 +0200},
	biburl    = {https://dblp.org/rec/conf/iclr/KipfW17.bib},
	bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{waniek2018hiding,
  title={Hiding individuals and communities in a social network},
  author={Waniek, Marcin and Michalak, Tomasz P and Wooldridge, Michael J and Rahwan, Talal},
  journal={Nature Human Behaviour},
  volume={2},
  number={2},
  pages={139--147},
  year={2018},
  publisher={Nature Publishing Group}
}

@inbook{zhou2018attacking,
	author = {Zhou, Kai and Michalak, Tomasz P. and Waniek, Marcin and Rahwan, Talal and Vorobeychik, Yevgeniy},
	title = {Attacking Similarity-Based Link Prediction in Social Networks},
	year = {2019},
	isbn = {9781450363099},
	publisher = {International Foundation for Autonomous Agents and Multiagent Systems},
	address = {Richland, SC},
	abstract = {Link prediction is one of the fundamental problems in computational social science.
	A particularly common means to predict existence of unobserved links is via structural
	similarity metrics, such as the number of common neighbors; node pairs with higher
	similarity are thus deemed more likely to be linked. However, a number of applications
	of link prediction, such as predicting links in gang or terrorist networks, are adversarial,
	with another party incentivized to minimize its effectiveness by manipulating observed
	information about the network. We offer a comprehensive algorithmic investigation
	of the problem of attacking similarity-based link prediction through link deletion,
	focusing on two broad classes of such approaches, one which uses only local information
	about target links, and another which uses global network information. While we show
	several variations of the general problem to be NP-Hard for both local and global
	metrics, we exhibit a number of well-motivated special cases which are tractable.
	Additionally, we provide principled and empirically effective algorithms for the intractable
	cases, in some cases proving worst-case approximation guarantees.},
	booktitle = {Proceedings of the 18th International Conference on Autonomous Agents and MultiAgent Systems},
	pages = {305–313},
	numpages = {9}
}

@inproceedings{li2020adversarial,
	title={Adversarial attack on community detection by hiding individuals},
	author={Li, Jia and Zhang, Honglei and Han, Zhichao and Rong, Yu and Cheng, Hong and Huang, Junzhou},
	booktitle={Proceedings of The Web Conference 2020},
	pages={917--927},
	year={2020}
}

@inproceedings{derr2018relevance,
  title={Relevance measurements in online signed social networks},
  author={Derr, Tyler and Wang, Chenxing and Wang, Suhang and Tang, Jiliang},
  booktitle={Proceedings of the 14th international workshop on mining and learning with graphs (MLG)},
  year={2018}
}

@article{tang2016survey,
  title={A survey of signed network mining in social media},
  author={Tang, Jiliang and Chang, Yi and Aggarwal, Charu and Liu, Huan},
  journal={ACM Computing Surveys (CSUR)},
  volume={49},
  number={3},
  pages={1--37},
  year={2016},
  publisher={ACM New York, NY, USA}
}


@inproceedings{zhu2019robust,
	title={Robust graph convolutional networks against adversarial attacks},
	author={Zhu, Dingyuan and Zhang, Ziwei and Cui, Peng and Zhu, Wenwu},
	booktitle={Proceedings of the 25th ACM SIGKDD International Conference on Knowledge Discovery \& Data Mining},
	pages={1399--1407},
	year={2019}
}

@inproceedings{jin2020graph,
	title={Graph structure learning for robust graph neural networks},
	author={Jin, Wei and Ma, Yao and Liu, Xiaorui and Tang, Xianfeng and Wang, Suhang and Tang, Jiliang},
	booktitle={Proceedings of the 26th ACM SIGKDD International Conference on Knowledge Discovery \& Data Mining},
	pages={66--74},
	year={2020}
}

@inproceedings{10.1145/3336191.3371789,
	author = {Entezari, Negin and Al-Sayouri, Saba A. and Darvishzadeh, Amirali and Papalexakis, Evangelos E.},
	title = {All You Need Is Low (Rank): Defending Against Adversarial Attacks on Graphs},
	year = {2020},
	isbn = {9781450368223},
	publisher = {Association for Computing Machinery},
	address = {New York, NY, USA},
	url = {https://doi.org/10.1145/3336191.3371789},
	doi = {10.1145/3336191.3371789},
	abstract = {Recent studies have demonstrated that machine learning approaches like deep learning
	methods are easily fooled by adversarial attacks. Recently, a highly-influential study
	examined the impact of adversarial attacks on graph data and demonstrated that graph
	embedding techniques are also vulnerable to adversarial attacks. Fake users on social
	media and fake product reviews are examples of perturbations in graph data that are
	realistic counterparts of the adversarial models proposed. Graphs are widely used
	in a variety of domains and it is highly important to develop graph analysis techniques
	that are robust to adversarial attacks. One of the recent studies on generating adversarial
	attacks for graph data is Nettack. The Nettack model has shown to be very successful
	in deceiving the Graph Convolutional Network (GCN) model. Nettack is also transferable
	to other node classification approaches e.g. node embeddings. In this paper, we explore
	the properties of Nettack perturbations, in search for effective defenses against
	them. Our first finding is that Nettack demonstrates a very specific behavior in the
	spectrum of the graph: only high-rank (low-valued) singular components of the graph
	are affected. Following that insight, we show that a low-rank approximation of the
	graph, that uses only the top singular components for its reconstruction, can greatly
	reduce the effects of Nettack and boost the performance of GCN when facing adversarial
	attacks. Indicatively, on the CiteSeer dataset, our proposed defense mechanism is
	able to reduce the success rate of Nettack from 98% to 36%. Furthermore, we show that
	tensor-based node embeddings, which by default project the graph into a low-rank subspace,
	are robust against Nettack perturbations. Lastly, we propose LowBlow, a low-rank adversarial
	attack which is able to affect the classification performance of both GCN and tensor-based
	node embeddings and we show that the low-rank attack is noticeable and making it unnoticeable
	results in a high-rank attack.},
	booktitle = {Proceedings of the 13th International Conference on Web Search and Data Mining},
	pages = {169–177},
	numpages = {9},
	keywords = {graph convolutional networks, graph mining, tensors, graph representation learning, adversarial machine learning},
	location = {Houston, TX, USA},
	series = {WSDM '20}
}


@InProceedings{deepsvdd,
	title = 	 {Deep One-Class Classification},
	author =       {Ruff, Lukas and Vandermeulen, Robert and Goernitz, Nico and Deecke, Lucas and Siddiqui, Shoaib Ahmed and Binder, Alexander and M{\"u}ller, Emmanuel and Kloft, Marius},
	booktitle = 	 {Proceedings of the 35th International Conference on Machine Learning},
	pages = 	 {4393--4402},
	year = 	 {2018},
	editor = 	 {Dy, Jennifer and Krause, Andreas},
	volume = 	 {80},
	series = 	 {Proceedings of Machine Learning Research},
	month = 	 {10--15 Jul},
	publisher =    {PMLR},
	pdf = 	 {http://proceedings.mlr.press/v80/ruff18a/ruff18a.pdf},
	url = 	 {https://proceedings.mlr.press/v80/ruff18a.html},
	abstract = 	 {Despite the great advances made by deep learning in many machine learning problems, there is a relative dearth of deep learning approaches for anomaly detection. Those approaches which do exist involve networks trained to perform a task other than anomaly detection, namely generative models or compression, which are in turn adapted for use in anomaly detection; they are not trained on an anomaly detection based objective. In this paper we introduce a new anomaly detection method—Deep Support Vector Data Description—, which is trained on an anomaly detection based objective. The adaptation to the deep regime necessitates that our neural network and training procedure satisfy certain properties, which we demonstrate theoretically. We show the effectiveness of our method on MNIST and CIFAR-10 image benchmark datasets as well as on the detection of adversarial examples of GTSRB stop signs.}
}


@inproceedings{graphsage,
	title={Inductive representation learning on large graphs},
	author={Hamilton, William L and Ying, Rex and Leskovec, Jure},
	booktitle={Proceedings of the 31st International Conference on Neural Information Processing Systems},
	pages={1025--1035},
	year={2017}
}

@article{relu,
	title={Deep learning using rectified linear units (relu)},
	author={Agarap, Abien Fred},
	journal={arXiv preprint arXiv:1803.08375},
	year={2018}
}

@inproceedings{zhang2018end,
	title={An end-to-end deep learning architecture for graph classification},
	author={Zhang, Muhan and Cui, Zhicheng and Neumann, Marion and Chen, Yixin},
	booktitle={Thirty-Second AAAI Conference on Artificial Intelligence},
	year={2018}
}

@inproceedings{10.1145/3219819.3219980,
	author = {Lee, John Boaz and Rossi, Ryan and Kong, Xiangnan},
	title = {Graph Classification Using Structural Attention},
	year = {2018},
	isbn = {9781450355520},
	publisher = {Association for Computing Machinery},
	address = {New York, NY, USA},
	url = {https://doi.org/10.1145/3219819.3219980},
	doi = {10.1145/3219819.3219980},
	pages = {1666–1674},
	numpages = {9},
	keywords = {attentional processing, deep learning, graph mining, reinforcement learning},
	location = {London, United Kingdom},
	series = {KDD '18}
}

@article{liben2007link,
	title={The link-prediction problem for social networks},
	author={Liben-Nowell, David and Kleinberg, Jon},
	journal={Journal of the American society for information science and technology},
	volume={58},
	number={7},
	pages={1019--1031},
	year={2007},
	publisher={Wiley Online Library}
}

@inproceedings{adam,
	author    = {Diederik P. Kingma and
	Jimmy Ba},
	editor    = {Yoshua Bengio and
	Yann LeCun},
	title     = {Adam: {A} Method for Stochastic Optimization},
	booktitle = {3rd International Conference on Learning Representations, {ICLR} 2015,
	San Diego, CA, USA, May 7-9, 2015, Conference Track Proceedings},
	year      = {2015},
	url       = {http://arxiv.org/abs/1412.6980},
	timestamp = {Thu, 25 Jul 2019 14:25:37 +0200},
	biburl    = {https://dblp.org/rec/journals/corr/KingmaB14.bib},
	bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{snea,
	title={Learning signed network embedding via graph attention},
	author={Li, Yu and Tian, Yuan and Zhang, Jiawei and Chang, Yi},
	booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
	volume={34},
	number={04},
	pages={4772--4779},
	year={2020}
}

@inproceedings{epinions,
	title={Trust management for the semantic web},
	author={Richardson, Matthew and Agrawal, Rakesh and Domingos, Pedro},
	booktitle={International semantic Web conference},
	pages={351--368},
	year={2003},
	organization={Springer}
}

@inproceedings{slashdot,
	title={Signed networks in social media},
	author={Leskovec, Jure and Huttenlocher, Daniel and Kleinberg, Jon},
	booktitle={Proceedings of the SIGCHI conference on human factors in computing systems},
	pages={1361--1370},
	year={2010}
}

@inproceedings{otc,
	title={Edge weight prediction in weighted signed networks},
	author={Kumar, Srijan and Spezzano, Francesca and Subrahmanian, VS and Faloutsos, Christos},
	booktitle={Data Mining (ICDM), 2016 IEEE 16th International Conference on},
	pages={221--230},
	year={2016},
	organization={IEEE}
}

@inproceedings{alpha,
	title={Rev2: Fraudulent user prediction in rating platforms},
	author={Kumar, Srijan and Hooi, Bryan and Makhija, Disha and Kumar, Mohit and Faloutsos, Christos and Subrahmanian, VS},
	booktitle={Proceedings of the Eleventh ACM International Conference on Web Search and Data Mining},
	pages={333--341},
	year={2018},
	organization={ACM}
}

@inproceedings{duan2014community,
	title={Community detection in graphs through correlation},
	author={Duan, Lian and Street, Willian Nick and Liu, Yanchi and Lu, Haibing},
	booktitle={Proceedings of the 20th ACM SIGKDD international conference on Knowledge discovery and data mining},
	pages={1376--1385},
	year={2014}
}

@inproceedings{xu2019topology,
	title = "Topology attack and defense for graph neural networks: An optimization perspective",
	abstract = "Graph neural networks (GNNs) which apply the deep neural networks to graph data have achieved significant performance for the task of semi-supervised node classification. However, only few work has addressed the adversarial robustness of GNNs. In this paper, we first present a novel gradient-based attack method that facilitates the difficulty of tackling discrete graph data. When comparing to current adversarial attacks on GNNs, the results show that by only perturbing a small number of edge perturbations, including addition and deletion, our optimization-based attack can lead to a noticeable decrease in classification performance. Moreover, leveraging our gradient-based attack, we propose the first optimization-based adversarial training for GNNs. Our method yields higher robustness against both different gradient based and greedy attack methods without sacrificing classification accuracy on original graph.",
	author = "Kaidi Xu and Hongge Chen and Sijia Liu and Chen, {Pin Yu} and Weng, {Tsui Wei} and Mingyi Hong and Xue Lin",
	note = "Funding Information: This work is supported by Air Force Research Laboratory FA8750-18-2-0058 and the MIT-IBM Watson AI Lab. Publisher Copyright: {\textcopyright} 2019 International Joint Conferences on Artificial Intelligence. All rights reserved.; 28th International Joint Conference on Artificial Intelligence, IJCAI 2019 ; Conference date: 10-08-2019 Through 16-08-2019",
	year = "2019",
	doi = "10.24963/ijcai.2019/550",
	language = "English (US)",
	series = "IJCAI International Joint Conference on Artificial Intelligence",
	publisher = "International Joint Conferences on Artificial Intelligence",
	pages = "3961--3967",
	editor = "Sarit Kraus",
	booktitle = "Proceedings of the 28th International Joint Conference on Artificial Intelligence, IJCAI 2019",
}

@article{fortunato2010community,
	title={Community detection in graphs},
	author={Fortunato, Santo},
	journal={Physics reports},
	volume={486},
	number={3-5},
	pages={75--174},
	year={2010},
	publisher={Elsevier}
}

@article{proteinsignednetwork,
	title={Integrating protein-protein interaction networks with phenotypes reveals signs of interactions},
	author={Vinayagam, Arunachalam and Zirin, Jonathan and Roesel, Charles and Hu, Yanhui and Yilmazel, Bahar and Samsonova, Anastasia A and Neum{\"u}ller, Ralph A and Mohr, Stephanie E and Perrimon, Norbert},
	journal={Nature methods},
	volume={11},
	number={1},
	pages={94--99},
	year={2014},
	publisher={Nature Publishing Group}
}

@article{stocksignednetwork,
	title={A network perspective of the stock market},
	author={Chi, K Tse and Liu, Jing and Lau, Francis CM},
	journal={Journal of Empirical Finance},
	volume={17},
	number={4},
	pages={659--667},
	year={2010},
	publisher={Elsevier}
}

@article{pei2020amalnet,
	title={AMalNet: A deep learning framework based on graph convolutional networks for malware detection},
	author={Pei, Xinjun and Yu, Long and Tian, Shengwei},
	journal={Computers \& Security},
	volume={93},
	pages={101792},
	year={2020},
	publisher={Elsevier}
}

@Inbook{Tsuda2010,
	author="Tsuda, Koji
	and Saigo, Hiroto",
	editor="Aggarwal, Charu C.
	and Wang, Haixun",
	title="Graph Classification",
	bookTitle="Managing and Mining Graph Data",
	year="2010",
	publisher="Springer US",
	address="Boston, MA",
	pages="337--363",
	abstract="Supervised learning on graphs is a central subject in graph data processing. In graph classification and regression, we assume that the target values of a certain number of graphs or a certain part of a graph are available as a training dataset, and our goal is to derive the target values of other graphs or the remaining part of the graph. In drug discovery applications, for example, a graph and its target value correspond to a chemical compound and its chemical activity. In this chapter, we review state-of-the-art methods of graph classification. In particular, we focus on two representative methods, graph kernels and graph boosting, and we present other methods in relation to the two methods. We describe the strengths and weaknesses of different graph classification methods and recent efforts to overcome the challenges.",
	isbn="978-1-4419-6045-0",
	doi="10.1007/978-1-4419-6045-0_11",
	url="https://doi.org/10.1007/978-1-4419-6045-0_11"
}

@inproceedings{
	mettack,
	title={Adversarial Attacks on Graph Neural Networks via Meta Learning},
	author={Daniel Zügner and Stephan Günnemann},
	booktitle={International Conference on Learning Representations},
	year={2019},
	url={https://openreview.net/forum?id=Bylnx209YX},
}

@inproceedings{sse,
	title={Spectral analysis of signed graphs for clustering, prediction and visualization},
	author={Kunegis, J{\'e}r{\^o}me and Schmidt, Stephan and Lommatzsch, Andreas and Lerner, J{\"u}rgen and De Luca, Ernesto W and Albayrak, Sahin},
	booktitle={Proceedings of the 2010 SIAM International Conference on Data Mining},
	pages={559--570},
	year={2010},
	organization={SIAM}
}

@inproceedings{sine,
	title={Signed network embedding in social media},
	author={Wang, Suhang and Tang, Jiliang and Aggarwal, Charu and Chang, Yi and Liu, Huan},
	booktitle={Proceedings of the 2017 SIAM international conference on data mining},
	pages={327--335},
	year={2017},
	organization={SIAM}
}

@inproceedings{meta,
	title={Model-agnostic meta-learning for fast adaptation of deep networks},
	author={Finn, Chelsea and Abbeel, Pieter and Levine, Sergey},
	booktitle={International Conference on Machine Learning},
	pages={1126--1135},
	year={2017},
	organization={PMLR}
}

@Inbook{ols,
	author="Zdaniuk, Bozena",
	editor="Michalos, Alex C.",
	title="Ordinary Least-Squares (OLS) Model",
	bookTitle="Encyclopedia of Quality of Life and Well-Being Research",
	year="2014",
	publisher="Springer Netherlands",
	address="Dordrecht",
	pages="4515--4517",
	isbn="978-94-007-0753-5",
	doi="10.1007/978-94-007-0753-5_2008",
	url="https://doi.org/10.1007/978-94-007-0753-5_2008"
}

@inproceedings{esp,
	author = {Leskovec, Jure and Huttenlocher, Daniel and Kleinberg, Jon},
	title = {Predicting Positive and Negative Links in Online Social Networks},
	year = {2010},
	isbn = {9781605587998},
	publisher = {Association for Computing Machinery},
	address = {New York, NY, USA},
	url = {https://doi.org/10.1145/1772690.1772756},
	doi = {10.1145/1772690.1772756},
	abstract = {We study online social networks in which relationships can be either positive (indicating relations such as friendship) or negative (indicating relations such as opposition or antagonism). Such a mix of positive and negative links arise in a variety of online settings; we study datasets from Epinions, Slashdot and Wikipedia. We find that the signs of links in the underlying social networks can be predicted with high accuracy, using models that generalize across this diverse range of sites. These models provide insight into some of the fundamental principles that drive the formation of signed links in networks, shedding light on theories of balance and status from social psychology; they also suggest social computing applications by which the attitude of one user toward another can be estimated from evidence provided by their relationships with other members of the surrounding social network.},
	booktitle = {Proceedings of the 19th International Conference on World Wide Web},
	pages = {641–650},
	numpages = {10},
	keywords = {signed networks, trust, status theory, structural balance, positive edges, distrust, negative edges},
	location = {Raleigh, North Carolina, USA},
	series = {WWW '10}
}

@article{SBT,
  title={Structural balance: a generalization of Heider's theory.},
  author={D. Cartwright and F. Harary},
  journal={Psychological review},
  year={1956},
  volume={63 5},
  pages={
          277-93
        }
}

@article{https://doi.org/10.1002/bs.3830020403,
author = {Harary, Frank},
title = {Structural duality},
journal = {Behavioral Science},
volume = {2},
number = {4},
pages = {255-265},
doi = {https://doi.org/10.1002/bs.3830020403},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/bs.3830020403},
eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1002/bs.3830020403},
abstract = {Abstract Charles L. Dodgson, the eminent Oxford mathematician, once expounded, in the form of a conversation between an egg and a seven-and-a-half-year-old girl, the interesting concept of an “unbirthday.” Conversely and perhaps complementarily, lexiphiles enjoy making lists of words like couth, plussed, ept, ebriety, peccable. Structural duality is, of course, more than whimsical playing with words, but it is concerned with such notions as contrastatus (versus status), antibalance (versus balance), and unliaison person (versus liaison person). It also involves the use of various kinds of graphs as a mathematical model, an approach whose value lies in the fact that it is not bound by physical units of measurement. The rigorous mathematical development of a duality theory may provide a source of fruitful concepts for behavioral science.},
year = {1957}
}

@inproceedings{word,
	title={Semantic word clusters using signed spectral clustering},
	author={Sedoc, Joao and Gallier, Jean and Foster, Dean and Ungar, Lyle},
	booktitle={Proceedings of the 55th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)},
	pages={939--949},
	year={2017}
}

@article{NORMAN197266,
title = {A derivation of a measure of relative balance for social structures and a characterization of extensive ratio systems},
journal = {Journal of Mathematical Psychology},
volume = {9},
number = {1},
pages = {66-91},
year = {1972},
issn = {0022-2496},
doi = {https://doi.org/10.1016/0022-2496(72)90006-5},
url = {https://www.sciencedirect.com/science/article/pii/0022249672900065},
author = {Robert Z Norman and Fred S Roberts},
abstract = {As an extension of the Heider and Cartwright-Harary theory of balance in social structures (signed digraphs), a measure of relative balance which is derived from some plausible axioms is needed. Such a measure should reflect the balance ordering, i.e., the relation ‘one social structure is more balanced than another’. Axioms for such a balance ordering are stated below in terms of the signed digraph representing the social structure as in the Cartwright-Harary theory. The axioms give rise to a measure which determines the balance ordering uniquely, subject to choice of a parameter f(m) which represents the relative importance of a semicycle of length m in the signed digraph. Special values of the parameter f(m) give rise to measures previously suggested as plausible in the literature. Techniques for estimating the values f(m) are described. A second axiomatization for the balance ordering is obtained by translating the requirements on balance into a typical problem of measurement theory in the Suppes-Zinnes sense. The resulting axioms define a so-called extensive ratio system.}
}

@misc{pelino2012class,
      title={Towards a class of complex networks models for conflict dynamics}, 
      author={Vinicio Pelino and Filippo Maimone},
      year={2012},
      eprint={1203.1394},
      archivePrefix={arXiv},
      primaryClass={physics.soc-ph}
}

@inproceedings{AG,
  title={Spectral Analysis of Signed Graphs for Clustering, Prediction and Visualization},
  author={J{\'e}r{\^o}me Kunegis and Stephan Schmidt and Andreas Lommatzsch and J. Lerner and E. W. D. Luca and S. Albayrak},
  booktitle={SDM},
  year={2010}
}

@article{FG,
author = {Aref, Samin and Mason, Andrew J. and Wilson, Mark C.},
title = {A modeling and computational study of the frustration index in signed networks},
journal = {Networks},
volume = {75},
number = {1},
pages = {95-110},
keywords = {0-1 integer linear programming, balance theory, binary programming, frustration index, line index of balance, optimization, signed graph, signed networks},
doi = {https://doi.org/10.1002/net.21907},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/net.21907},
eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1002/net.21907},
abstract = {Abstract Computing the frustration index of a signed graph is a key step toward solving problems in many fields including social networks, political science, physics, chemistry, and biology. The frustration index determines the distance of a network from a state of total structural balance. Although the definition of the frustration index goes back to the 1950s, its exact algorithmic computation, which is closely related to classic NP-hard graph problems, has only become a focus in recent years. We develop three new binary linear programming models to compute the frustration index exactly and efficiently as the solution to a global optimization problem. Solving the models with prioritized branching and valid inequalities in Gurobi, we can compute the frustration index of real signed networks with over 15 000 edges in less than a minute on inexpensive hardware. We provide extensive performance analysis for both random and real signed networks and show that our models outperform all existing approaches by large factors. Based on resolution time, algorithm output, and effective branching factor we highlight the superiority of our models to both exact and heuristic methods in the literature.},
year = {2020}
}

@article{FI1,
author = {Aref, Samin and Mason, Andrew J. and Wilson, Mark C.},
title = {A modeling and computational study of the frustration index in signed networks},
journal = {Networks},
volume = {75},
number = {1},
pages = {95-110},
keywords = {0-1 integer linear programming, balance theory, binary programming, frustration index, line index of balance, optimization, signed graph, signed networks},
doi = {https://doi.org/10.1002/net.21907},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/net.21907},
eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1002/net.21907},
abstract = {Abstract Computing the frustration index of a signed graph is a key step toward solving problems in many fields including social networks, political science, physics, chemistry, and biology. The frustration index determines the distance of a network from a state of total structural balance. Although the definition of the frustration index goes back to the 1950s, its exact algorithmic computation, which is closely related to classic NP-hard graph problems, has only become a focus in recent years. We develop three new binary linear programming models to compute the frustration index exactly and efficiently as the solution to a global optimization problem. Solving the models with prioritized branching and valid inequalities in Gurobi, we can compute the frustration index of real signed networks with over 15 000 edges in less than a minute on inexpensive hardware. We provide extensive performance analysis for both random and real signed networks and show that our models outperform all existing approaches by large factors. Based on resolution time, algorithm output, and effective branching factor we highlight the superiority of our models to both exact and heuristic methods in the literature.},
year = {2020}
}

@Inbook{Aref2018,
author="Aref, Samin
and Mason, Andrew J.
and Wilson, Mark C.",
editor="Goldengorin, Boris",
title="Computing the Line Index of Balance Using Integer Programming Optimisation",
bookTitle="Optimization Problems in Graph Theory: In Honor of Gregory Z. Gutin's 60th Birthday",
year="2018",
publisher="Springer International Publishing",
address="Cham",
pages="65--84",
abstract="An important measure of signed graphs is the line index of balance which has applications in many fields. However, this graph-theoretic measure was underused for decades because of the inherent complexity in its computation which is closely related to solving NP-hard graph optimisation problems like MAXCUT. We develop new quadratic and linear programming models to compute the line index of balance exactly. Using the Gurobi integer programming optimisation solver, we evaluate the line index of balance on real-world and synthetic datasets. The synthetic data involves Erd{\H{o}}s-R{\'e}nyi graphs, Barab{\'a}si-Albert graphs, and specially structured random graphs. We also use well-known datasets from the sociology literature, such as signed graphs inferred from students' choice and rejection, as well as datasets from the biology literature including gene regulatory networks. The results show that exact values of the line index of balance in relatively large signed graphs can be efficiently computed using our suggested optimisation models. We find that most real-world social networks and some biological networks have a small line index of balance which indicates that they are close to balanced.",
isbn="978-3-319-94830-0",
doi="10.1007/978-3-319-94830-0_3",
url="https://doi.org/10.1007/978-3-319-94830-0_3"
}

@INPROCEEDINGS{sgcn,
  author={Derr, Tyler and Ma, Yao and Tang, Jiliang},
  booktitle={2018 IEEE International Conference on Data Mining (ICDM)}, 
  title={Signed Graph Convolutional Networks}, 
  year={2018},
  volume={},
  number={},
  pages={929-934},
  doi={10.1109/ICDM.2018.00113}}

@inproceedings{nettack,
	author = {Z\"{u}gner, Daniel and Akbarnejad, Amir and G\"{u}nnemann, Stephan},
	title = {Adversarial Attacks on Neural Networks for Graph Data},
	year = {2018},
	isbn = {9781450355520},
	publisher = {Association for Computing Machinery},
	address = {New York, NY, USA},
	url = {https://doi.org/10.1145/3219819.3220078},
	doi = {10.1145/3219819.3220078},
	pages = {2847–2856},
	numpages = {10},
	keywords = {adversarial machine learning, graph convolutional networks, network mining, graph mining, semi-supervised learning},
	location = {London, United Kingdom},
	series = {KDD '18}
}

@inproceedings{diffpool,
	author = {Ying, Rex and You, Jiaxuan and Morris, Christopher and Ren, Xiang and Hamilton, William L. and Leskovec, Jure},
	title = {Hierarchical Graph Representation Learning with Differentiable Pooling},
	year = {2018},
	publisher = {Curran Associates Inc.},
	address = {Red Hook, NY, USA},
	abstract = {Recently, graph neural networks (GNNs) have revolutionized the field of graph representation
	learning through effectively learned node embeddings, and achieved state-of-the-art
	results in tasks such as node classification and link prediction. However, current
	GNN methods are inherently flat and do not learn hierarchical representations of graphs—a
	limitation that is especially problematic for the task of graph classification, where
	the goal is to predict the label associated with an entire graph. Here we propose
	DIFFPOOL, a differentiable graph pooling module that can generate hierarchical representations
	of graphs and can be combined with various graph neural network architectures in an
	end-to-end fashion. DIFFPOOL learns a differentiable soft cluster assignment for nodes
	at each layer of a deep GNN, mapping nodes to a set of clusters, which then form the
	coarsened input for the next GNN layer. Our experimental results show that combining
	existing GNN methods with DIFFPOOL yields an average improvement of 5-10% accuracy
	on graph classification benchmarks, compared to all existing pooling approaches, achieving
	a new state-of-the-art on four out of five benchmark data sets.},
	booktitle = {Proceedings of the 32nd International Conference on Neural Information Processing Systems},
	pages = {4805–4815},
	numpages = {11},
	location = {Montr\'{e}al, Canada},
	series = {NIPS'18}
}

@inproceedings{SAGpool,
	title={Self-attention graph pooling},
	author={Lee, Junhyun and Lee, Inyeop and Kang, Jaewoo},
	booktitle={International Conference on Machine Learning},
	pages={3734--3743},
	year={2019},
	organization={PMLR}
}
